Taming Video Diffusion Prior with Scene-Grounding Guidance for 3D Gaussian Splatting from Sparse Inputs

Despite recent successes in novel view synthesis using 3D Gaussian Splatting (3DGS), modeling scenes with sparse inputs remains a challenge. In this work, we address two critical yet overlooked issues in real-world sparse-input modeling: extrapolation and occlusion. To tackle these issues, we propose to use a reconstruction by generation pipeline that leverages learned priors from video diffusion models to provide plausible interpretations for regions outside the field of view or occluded. However, the generated sequences exhibit inconsistencies that do not fully benefit subsequent 3DGS modeling. To address the challenge of inconsistencies, we introduce a novel scene-grounding guidance based on rendered sequences from an optimized 3DGS, which tames the diffusion model to generate consistent sequences. This guidance is training-free and does not require any fine-tuning of the diffusion model. To facilitate holistic scene modeling, we also propose a trajectory initialization method. It effectively identifies regions that are outside the field of view and occluded. We further design a scheme tailored for 3DGS optimization with generated sequences. Experiments demonstrate that our method significantly improves upon the baseline and achieves state-of-the-art performance on challenging benchmarks.

==> sec/teaser.tex <==
\begin{figure}
\vspace{-4mm}
\twocolumn[{%
\renewcommand\twocolumn[1][]{#1}%
\maketitle
\centering
% \setlength\tabcolsep{0pt}
% \vspace{-12pt}
\includegraphics[width=0.98\linewidth]{images/teaser}
\vspace{-8pt}
\captionof{figure}{We tackle the critical issues of \textbf{(a) extrapolation and (b) occlusion} in sparse-input 3DGS by leveraging a video diffusion model. Vanilla generation often suffers from inconsistencies within the generated sequences (as highlighted by the yellow arrows), leading to black shadows in the rendered images. In contrast, our scene-grounding generation produces consistent sequences, effectively addressing these issues and enhancing overall quality (c), as indicated by the blue boxes. The numbers refer to PSNR values. Zoom in for better~visualization. 
}\vspace{2mm}\label{fig:teaser}
}]
\end{figure}
